Hate Speech Criteria: A Modular Approach to Task-Specific Hate Speech Definitions

\textbf{Offensive Content Warning}: This paper contains offensive language only for providing examples that clarify this research and do not reflect the authors' opinions. Please be aware that these examples are offensive and may cause you distress. The subjectivity of recognizing \textit{hate speech} makes it a complex task. This is also reflected by different and incomplete definitions in NLP. We present \textit{hate speech} criteria, developed with perspectives from law and social science, with the aim of helping researchers create more precise definitions and annotation guidelines on five aspects: (1) target groups, (2) dominance, (3) perpetrator characteristics, (4) type of negative group reference, and the (5) type of potential consequences/effects. Definitions can be structured so that they cover a more broad or more narrow phenomenon. As such, conscious choices can be made on specifying criteria or leaving them open. We argue that the goal and exact task developers have in mind should determine how the scope of \textit{hate speech} is defined. We provide an overview of the properties of English datasets from \url{hatespeechdata.com} that may help select the most suitable dataset for a specific scenario.

==> tables/definitions_table.tex <==
\begin{table*}[h!]
%     \centering
    \begin{tabular}{cp{10.5cm}}
        \toprule
        \textbf{Paper}  &  \textbf{Definition}  \\
        \midrule  
        \citet{schmidt-wiegand-2017-survey} & \textit{Hate speech} is commonly defined as any communication that disparages a person or a group on the basis of some characteristic such as race, color, ethnicity, gender, sexual orientation, nationality, religion, or other characteristic \citep{nockleby}   \\
        \midrule
        \citet{davidson2017automated}  & \textit{Hate speech} is defined as language that is used to express hatred towards a targeted group or is intended to be derogatory, to humiliate, or to insult the members of the group. May also be language that threatens or incites violence \\
        \midrule
        \citet{founta2018large} & Language used to express hatred towards a targeted individual or group, or is intended to be derogatory, to humiliate, or to insult the members of the group, on the basis of attributes such as race, religion, ethnic origin, sexual orientation, disability, or gender. \\ 
        \midrule 
        \citet{talat-hovy-2016-hateful} & \begin{enumerate}
            \item uses a sexist or racial slurs
            \item attacks a minority.
            \item seeks to silence a minority.
            \item criticizes a minority (without a well founded argument).
            \item promotes, but does not directly use, hate speech or violent crime.
            \item criticizes a minority and uses a straw man argument.
            \item blatantly misrepresents truth or seeks to distort views on a minority with unfounded claims.
            \item shows support of problematic hash tags. E.g. “\#BanIslam”, “\#whoriental”, “\#whitegenocide”
            \item negatively stereotypes a minority.
            \item defends xenophobia or sexism.
            \item contains a screen name that is offensive, as per the previous criteria, the tweet is ambiguous (at best), and the tweet is on a topic that satisfies any of the above criteria.
        \end{enumerate} \\
        \bottomrule
    \end{tabular}
    \caption{Different papers/datasets and their definition.}
    \label{tab:definitions}
\end{table*}
